Approval Voting in Product Societies

In approval voting, individuals vote for all platforms that they find acceptable. In this situation it is natural to ask: When is agreement possible? What conditions guarantee that some fraction of the voters agree on even a single platform? Berg et. al. found such conditions when voters are asked to make a decision on a single issue that can be represented on a linear spectrum. In particular, they showed that if two out of every three voters agree on a platform, there is a platform that is acceptable to a majority of the voters. Hardin developed an analogous result when the issue can be represented on a circular spectrum. We examine scenarios in which voters must make two decisions simultaneously. For example, if voters must decide on the day of the week to hold a meeting and the length of the meeting, then the space of possible options forms a cylindrical spectrum. Previous results do not apply to these multi-dimensional voting societies because a voter's preference on one issue often impacts their preference on another. We present a general lower bound on agreement in a two-dimensional voting society, and then examine specific results for societies whose spectra are cylinders and tori.

==> stratified_figure.tex <==
 \begin{tikzpicture}[scale=0.7]
    	%parameters
    	\def\a{1}	%minor radius
        \def\b{2}	%major radius
        \def\t{0.5} %thickness of preference bands
        \def\s{2.5} %thickness of strata
        
        %background arcs
        \foreach \i in {1,2,3,4}
        {
            \draw[thick,dashed,gray] (\s*\i, \b) arc(90:270:{\a} and {\b});
        }
        
        %shading for other strata
        \fill[lightgray,fill opacity=0.5] (\s,\b) arc(90:-90:{\a} and {\b}) -- (4*\s,-\b) arc(-90:90:{\a} and {\b}) -- cycle;
        \fill[lightgray,fill opacity=0.3] (\s,\b) arc(90:270:{\a} and {\b}) -- (4*\s,-\b) arc(270:90:{\a} and {\b}) -- cycle;
        
        %left strata
        \draw[black!60!green,fill=green,fill opacity=0.5] (\a+\t,0) arc(0:90:{\a} and {\b}) -- (4*\t,\b) arc(90:0:{\a} and {\b}) -- cycle;
        \draw[black!60!green,dashed,fill=green,fill opacity=0.3] (-\a+\t,0) arc(180:90:{\a} and {\b}) -- (4*\t,\b) arc(90:180:{\a} and {\b}) -- cycle;
        
        \draw[black!60!blue,fill=blue,fill opacity=0.5] (0.5*\t,-\b) arc(-90:30:{\a} and {\b}) -- (5*\t,0.5*\b) arc(30:-90:{\a} and {\b}) -- cycle;
        \draw[black!60!blue,dashed,fill=blue,fill opacity=0.3] (0.5*\t,-\b) arc(270:210:{\a} and {\b}) -- (1.5*\t,-0.5*\b) arc(210:270:{\a} and {\b}) -- cycle;
        
        \draw[black!60!red,fill=red,fill opacity=0.5] (1.5*\t,-\b) arc(270:330:{\a} and {\b}) -- (5.5*\t,-0.5*\b) arc(330:270:{\a} and {\b}) -- cycle;
        \draw[black!60!red,dashed,fill=red,fill opacity=0.3] (1.5*\t,-\b) arc(270:150:{\a} and {\b}) -- (2*\t,0.5*\b) arc(150:270:{\a} and {\b}) -- cycle;
        
     	%foreground cylinder
		\draw[thick] (0,0) ellipse ({\a} and \b);
        \foreach \i in {1,2,3,4}
        {
            \draw[thick] (\s*\i,-1*\b) arc(-90:90:{\a} and {\b});

        }
        \draw[thick] (0,-1*\b) -- (10,-1*\b);
        \draw[thick] (0,\b) -- (10,\b);
        
        %brackets
        \draw [decorate,decoration={brace,amplitude=8pt},xshift=0pt,yshift=-6pt]
(5*\t,-\b) -- (0,-\b) node [black,midway,yshift=-14pt] {one strata};
\end{tikzpicture}

==> torus_fig_1.tex <==
\begin{tikzpicture}
	%rectangles
    \fill[purple,opacity=0.5] (0.2,0.2) rectangle (2.8,2.8);
    \fill[blue,opacity=0.5] (1.2,2.2) rectangle (3.8,4.8);
    \fill[green,opacity=0.5] (2.2,0) rectangle (4.8,1.8);
    \fill[green,opacity=0.5] (2.2,4.2) rectangle (4.8,5);
    \fill[orange,opacity=0.5] (3.2,1.2) rectangle (5,3.8);
    \fill[orange,opacity=0.5] (0,1.2) rectangle (0.8,3.8);
    \fill[red,opacity=0.5] (4.2,3.2) rectangle (5,5);
    \fill[red,opacity=0.5] (0,0) rectangle (1.8,0.8);
    \fill[red,opacity=0.5] (0,3.2) rectangle (1.8,5);
    \fill[red,opacity=0.5] (4.2,0) rectangle (5,0.8);
   	
    %torus border
    \draw (0,0) rectangle (5,5);

	%horizontal labels
	\draw[purple] (0.2,-0.1) -- +(0,-0.3);
    \draw[purple] (0.2,-0.25) -- +(0.15,0);
    \node[purple] at (0.4,-0.5) {$A$};
    
    \draw[orange] (0.8,-0.1) -- +(0,-0.3);
    \draw[orange] (0.8,-0.25) -- +(-0.15,0);
    \node[orange] at (0.95,-0.5) {$B$};
    
    \draw[blue] (1.2,-0.1) -- +(0,-0.3);
    \draw[blue] (1.2,-0.25) -- +(0.15,0);
    \node[blue] at (1.4,-0.5) {$C$};
    
    \draw[red] (1.8,-0.1) -- +(0,-0.3);
    \draw[red] (1.8,-0.25) -- +(-0.15,0);
    \node[red] at (1.95,-0.5) {$D$};
    
    \draw[green] (2.2,-0.1) -- +(0,-0.3);
    \draw[green] (2.2,-0.25) -- +(0.15,0);
    \node[green] at (2.4,-0.5) {$E$};
    
    \draw[purple] (2.8,-0.1) -- +(0,-0.3);
    \draw[purple] (2.8,-0.25) -- +(-0.15,0);
    \node[purple] at (2.95,-0.5) {$A$};
    
    \draw[orange] (3.2,-0.1) -- +(0,-0.3);
    \draw[orange] (3.2,-0.25) -- +(0.15,0);
    \node[orange] at (3.4,-0.5) {$B$};
    
    \draw[blue] (3.8,-0.1) -- +(0,-0.3);
    \draw[blue] (3.8,-0.25) -- +(-0.15,0);
    \node[blue] at (3.95,-0.5) {$C$};
    
    \draw[red] (4.2,-0.1) -- +(0,-0.3);
    \draw[red] (4.2,-0.25) -- +(0.15,0);
    \node[red] at (4.4,-0.5) {$D$};
    
    \draw[green] (4.8,-0.1) -- +(0,-0.3);
    \draw[green] (4.8,-0.25) -- +(-0.15,0);
    \node[green] at (4.95,-0.5) {$E$};
    
    %vertical labels
    \draw[purple] (-0.3,0.2) -- +(-0.3,0);
    \draw[purple] (-0.45,0.2) -- +(0,0.15);
    \node[purple] at (-0.2,0.1) {$A$};
    
    \draw[red] (-0.3,0.8) -- +(-0.3,0);
    \draw[red] (-0.45,0.8) -- +(0,-0.15);
    \node[red] at (-0.2,0.6) {$D$};
    
    \draw[orange] (-0.3,1.2) -- +(-0.3,0);
    \draw[orange] (-0.45,1.2) -- +(0,0.15);
    \node[orange] at (-0.2,1.1) {$B$};
    
    \draw[green] (-0.3,1.8) -- +(-0.3,0);
    \draw[green] (-0.45,1.8) -- +(0,-0.15);
    \node[green] at (-0.2,1.6) {$E$};
    
    \draw[blue] (-0.3,2.2) -- +(-0.3,0);
    \draw[blue] (-0.45,2.2) -- +(0,0.15);
    \node[blue] at (-0.2,2.1) {$C$};
    
    \draw[purple] (-0.3,2.8) -- +(-0.3,0);
    \draw[purple] (-0.45,2.8) -- +(0,-0.15);
    \node[purple] at (-0.2,2.6) {$A$};
    
    \draw[red] (-0.3,3.2) -- +(-0.3,0);
    \draw[red] (-0.45,3.2) -- +(0,0.15);
    \node[red] at (-0.2,3.1) {$D$};
    
    \draw[orange] (-0.3,3.8) -- +(-0.3,0);
    \draw[orange] (-0.45,3.8) -- +(0,-0.15);
    \node[orange] at (-0.2,3.6) {$B$};
    
    \draw[green] (-0.3,4.2) -- +(-0.3,0);
    \draw[green] (-0.45,4.2) -- +(0,0.15);
    \node[green] at (-0.2,4.1) {$E$};
    
    \draw[blue] (-0.3,4.8) -- +(-0.3,0);
    \draw[blue] (-0.45,4.8) -- +(0,-0.15);
    \node[blue] at (-0.2,4.6) {$C$};
\end{tikzpicture}
